GraphCliff: Short-Long Range Gating for Modeling Critical Activity Changes Caused by Subtle Molecular Differences

The quantitative structure-activity relationship assumes a smooth mapping between molecular structure and biological activity. However, activity cliffs, defined as pairs of structurally similar compounds with large potency differences, break this continuity. Recent activity cliff benchmarks show that machine learning models with extended connectivity fingerprints outperform graph neural networks. Our analysis shows that the embedding distances of conventional graph neural networks fail to reflect the activity differences, collapsing structurally similar yet functionally divergent molecules into nearly indistinguishable representations. To recover sensitivity to such local changes while preserving global molecular context, we propose GraphCliff, which integrates short and long range information at the node level through a locally conditioned gating mechanism. Experimental results demonstrate that GraphCliff consistently improves performance on both non-cliff and cliff compounds, with layer-wise embedding analyses attributing these gains to sharper discrimination of structurally similar molecules relative to strong baseline graph models.

==> tables/full_results1.tex <==
%\begin{landscape}

\begin{table}[htbp]
\centering
\caption{RMSE / $\text{RMSE}_{\text{cliff}}$ (Part 1/3) with best (\textbf{bold}) and second-best (\underline{underlined}) highlighted.}
\scalebox{0.73}{%

\begin{tabular}{llcccccccccc}
\toprule
\textbf{Algorithm} & \textbf{Descriptor} & \textbf{CHEMBL1862} & \textbf{CHEMBL1871} & \textbf{CHEMBL2034} & \textbf{CHEMBL2047} & \textbf{CHEMBL204} & \textbf{CHEMBL2147} & \textbf{CHEMBL214} & \textbf{CHEMBL218} & \textbf{CHEMBL219} & \textbf{CHEMBL228} \\
& & \textbf{(Ki)} & \textbf{(Ki)} & \textbf{(Ki)} & \textbf{(EC50)} & \textbf{(Ki)} & \textbf{(Ki)} & \textbf{(Ki)} & \textbf{(EC50)} & \textbf{(Ki)} & \textbf{(Ki)} \\
\midrule

GraphCliff & GRAPH & 0.7810 / \underline{0.6740} & \underline{0.6279} / 0.7975 & 0.7473 / 0.8580 & \underline{0.5924} / 0.6549 & \textbf{0.6914} / \textbf{0.8212} & \underline{0.5600} / \textbf{0.5790} & \textbf{0.6210} / \underline{0.7260} & 0.6974 / 0.7811 & \underline{0.6636} / \underline{0.7435} & \textbf{0.6513} / \textbf{0.6739} \\
GraphCliff w/ JK-Net & GRAPH & 0.8194 / 0.7496 & \textbf{0.6042} / \textbf{0.7342} & 0.7718 / 0.9196 & 0.6289 / 0.7330 & \underline{0.6947} / \underline{0.8226} & \textbf{0.5581} / 0.6186 & \underline{0.6302} / 0.7485 & 0.7252 / 0.7997 & \textbf{0.6634} / \textbf{0.7328} & 0.6672 / 0.6902 \\
SVM & ECFP & \underline{0.7736} / \textbf{0.6739} & 0.6649 / 0.8734 & \textbf{0.6737} / \textbf{0.8129} & 0.6136 / 0.6874 & 0.7231 / 0.8588 & 0.5762 / \underline{0.5796} & 0.6345 / \textbf{0.7238} & 0.7190 / 0.7614 & 0.7096 / 0.7883 & \underline{0.6621} / \underline{0.6759} \\
GraphCLiff w/ Residual & GRAPH & 0.8148 / 0.7696 & 0.6615 / \underline{0.7796} & 0.7369 / 0.8556 & 0.6177 / 0.6779 & 0.7126 / 0.8479 & 0.5815 / 0.6362 & 0.6415 / 0.7612 & 0.7669 / 0.8055 & 0.7052 / 0.7818 & 0.7010 / 0.6994 \\
GBM & ECFP & 0.7977 / 0.7465 & 0.6775 / 0.9221 & 0.7674 / 0.8637 & 0.6020 / 0.6396 & 0.7533 / 0.9320 & 0.5811 / 0.6161 & 0.6775 / 0.7611 & 0.7116 / 0.7464 & 0.7117 / 0.7646 & 0.6862 / 0.7234 \\
RF & ECFP & 0.8051 / 0.6859 & 0.6600 / 0.9064 & 0.7269 / 0.8518 & 0.6275 / 0.6646 & 0.7628 / 0.8988 & 0.6616 / 0.6763 & 0.7003 / 0.8010 & 0.7055 / 0.7596 & 0.7227 / 0.7650 & 0.7093 / 0.7733 \\
GINE + PairNorm & GRAPH & 0.8408 / 0.7460 & 0.6301 / 0.8670 & 0.7245 / 0.8453 & 0.6125 / \underline{0.5953} & 0.7451 / 0.8983 & 0.6933 / 0.6793 & 0.7222 / 0.8089 & \underline{0.6903} / 0.7711 & 0.7198 / 0.7691 & 0.6931 / 0.7139 \\
JK-Net & GRAPH & 0.9715 / 0.9612 & 0.6400 / 0.8227 & 0.7143 / \underline{0.8245} & \textbf{0.5921} / \textbf{0.5779} & 0.7783 / 0.8997 & 0.6663 / 0.6807 & 0.6665 / 0.7683 & 0.7348 / 0.7825 & 0.7400 / 0.8127 & 0.7129 / 0.7710 \\
GINE + NodeNorm & GRAPH & 0.9213 / 0.8562 & 0.6720 / 0.8341 & 0.7187 / 0.8524 & 0.6542 / 0.7203 & 0.7376 / 0.8635 & 0.7788 / 0.6964 & 0.6806 / 0.7934 & 0.7653 / 0.7763 & 0.7021 / 0.7969 & 0.7017 / 0.7565 \\
GINE + Residual & GRAPH & 0.8660 / 0.7848 & 0.6778 / 0.7810 & 0.7300 / 0.8964 & 0.6696 / 0.6731 & 0.8000 / 0.9378 & 0.7111 / 0.7330 & 0.7098 / 0.8114 & 0.7265 / 0.7927 & 0.7472 / 0.8188 & 0.7080 / 0.7927 \\
KNN & ECFP & 0.8983 / 0.8218 & 0.6498 / 0.8170 & 0.6965 / 0.9133 & 0.6418 / 0.7353 & 0.8207 / 0.9954 & 0.6618 / 0.6821 & 0.7335 / 0.8742 & 0.7355 / 0.7848 & 0.7754 / 0.8159 & 0.7173 / 0.8112 \\
ChemProp & GRAPH & 0.8149 / 0.6928 & 0.7043 / 0.9193 & 0.7748 / 0.8857 & 0.6933 / 0.7203 & 0.8109 / 0.8506 & 0.6491 / 0.6392 & 0.6600 / 0.8247 & 0.7580 / 0.7938 & 0.6916 / 0.7740 & 0.6705 / 0.6951 \\
LSTM & SMILES & \textbf{0.7614} / 0.7927 & 0.6621 / 0.8502 & 0.7553 / 0.9441 & 0.6955 / 0.7904 & 0.8224 / 0.9302 & 0.6465 / 0.7246 & 0.7232 / 0.8506 & 0.7479 / 0.8178 & 0.7797 / 0.8549 & 0.7788 / 0.8836 \\
GBM & MACCS & 0.8602 / 0.7781 & 0.6859 / 0.9039 & 0.7234 / 0.8565 & 0.6703 / 0.7019 & 0.7998 / 0.9579 & 0.7915 / 0.7775 & 0.7295 / 0.8565 & 0.7152 / 0.7655 & 0.8159 / 0.8619 & 0.7701 / 0.8074 \\
SVM & MACCS & 0.8905 / 0.8592 & 0.6702 / 0.8905 & \underline{0.6808} / 0.8602 & 0.6947 / 0.7363 & 0.8059 / 0.9832 & 0.7937 / 0.8061 & 0.7463 / 0.8888 & 0.7030 / \underline{0.7289} & 0.8204 / 0.8839 & 0.7450 / 0.7924 \\
RF & MACCS & 0.8739 / 0.8439 & 0.7025 / 0.9044 & 0.7002 / 0.8283 & 0.6765 / 0.7071 & 0.8149 / 0.9706 & 0.8060 / 0.7925 & 0.7467 / 0.8872 & \textbf{0.6688} / \textbf{0.7124} & 0.8070 / 0.8375 & 0.7690 / 0.8097 \\
MLP & ECFP & 0.8776 / 0.7811 & 0.7367 / 0.9579 & 0.7423 / 0.8488 & 0.6766 / 0.7283 & 0.8154 / 0.9622 & 0.7232 / 0.7035 & 0.6932 / 0.7803 & 0.7851 / 0.8059 & 0.7557 / 0.8319 & 0.7550 / 0.7574 \\
GINE + DropEdge & GRAPH & 1.0060 / 0.9994 & 0.7704 / 0.9536 & 0.7485 / 0.9009 & 0.7415 / 0.7301 & 0.8658 / 0.9784 & 0.7846 / 0.8020 & 0.7644 / 0.8741 & 0.8521 / 0.8753 & 0.8325 / 0.8942 & 0.8104 / 0.8577 \\
SCAGE & GRAPH & 0.8753 / 0.6768 & 0.7582 / 0.8230 & 0.7446 / 0.8250 & 0.7137 / 0.6054 & 0.8135 / 0.8884 & 0.9104 / 0.8584 & 0.7793 / 0.8336 & 0.7379 / 0.7833 & 0.8765 / 0.8630 & 0.7713 / 0.7865 \\
GCNII & GRAPH & 0.9601 / 0.9193 & 0.7403 / 0.9383 & 0.7593 / 0.8566 & 0.7248 / 0.7001 & 0.8258 / 0.9342 & 1.0474 / 0.9713 & 0.7543 / 0.8342 & 0.7576 / 0.8331 & 0.8156 / 0.8606 & 0.7838 / 0.8280 \\
KNN & MACCS & 1.0494 / 0.8676 & 0.7051 / 0.9412 & 0.7682 / 0.9102 & 0.7057 / 0.6895 & 0.8910 / 1.0433 & 0.9438 / 0.8668 & 0.7988 / 0.9017 & 0.7071 / 0.7560 & 0.8726 / 0.8878 & 0.7785 / 0.8362 \\
APPNP & GRAPH & 1.0084 / 0.9476 & 0.7624 / 0.9685 & 0.7650 / 0.8998 & 0.7595 / 0.7709 & 0.8719 / 0.9734 & 1.1075 / 1.0046 & 0.8000 / 0.8887 & 0.8527 / 0.8863 & 0.8865 / 0.9236 & 0.8442 / 0.8787 \\
RF & PHYSCHEM & 0.9085 / 0.9395 & 0.7530 / 1.0577 & 0.7054 / 0.8348 & 0.8137 / 0.9004 & 1.1046 / 1.1609 & 0.9720 / 0.9162 & 0.9090 / 0.9892 & 0.8228 / 0.7997 & 0.9297 / 0.9700 & 0.9214 / 0.9166 \\
GBM & PHYSCHEM & 0.9427 / 0.9033 & 0.7244 / 1.0485 & 0.7292 / 0.8670 & 0.8130 / 0.9096 & 1.1445 / 1.2108 & 0.9486 / 0.8935 & 0.8949 / 0.9881 & 0.8286 / 0.8262 & 0.9496 / 0.9798 & 0.9072 / 0.9228 \\
Transformer & TOKENS & 0.9606 / 0.9637 & 0.8085 / 1.0729 & 0.8036 / 0.9380 & 0.7667 / 0.7253 & 1.0979 / 1.2547 & 0.9026 / 0.8930 & 0.8617 / 0.9523 & 0.8692 / 0.8951 & 0.8781 / 0.9398 & 0.9076 / 0.9787 \\
GCN & GRAPH & 0.9416 / 0.9420 & 0.7689 / 1.0090 & 0.8100 / 0.9282 & 0.7973 / 0.7807 & 1.0563 / 1.2010 & 0.8400 / 0.8251 & 1.0068 / 1.0836 & 0.9276 / 0.9518 & 1.0263 / 1.0553 & 0.9583 / 1.0005 \\
KNN & PHYSCHEM & 1.0008 / 0.9602 & 0.7969 / 1.0635 & 0.7609 / 0.9014 & 0.7655 / 0.8450 & 1.1148 / 1.1689 & 1.0530 / 0.9226 & 0.9710 / 1.0487 & 0.8828 / 0.8324 & 0.9701 / 0.9853 & 0.9893 / 0.9343 \\
CNN & SMILES & 1.0489 / 0.8998 & 0.8100 / 1.0410 & 0.7978 / 0.9335 & 0.7761 / 0.7740 & 1.1314 / 1.2338 & 0.9246 / 0.9338 & 0.9310 / 1.0071 & 0.9584 / 0.9338 & 0.9768 / 0.9726 & 0.9652 / 0.9440 \\
SVM & PHYSCHEM & 0.9663 / 0.9201 & 0.8026 / 1.0663 & 0.7632 / 0.9102 & 0.7146 / 0.6672 & 1.2052 / 1.3129 & 0.9655 / 0.9065 & 0.9567 / 0.9649 & 1.0259 / 1.0046 & 0.9602 / 1.0090 & 0.9297 / 0.8905 \\
GAT & GRAPH & 0.9869 / 1.0007 & 0.7984 / 1.0424 & 0.8091 / 0.9415 & 0.8403 / 0.7896 & 1.1377 / 1.2815 & 0.9661 / 0.9167 & 1.0510 / 1.1372 & 0.9569 / 0.9835 & 0.9790 / 0.9824 & 1.0265 / 1.0278 \\
RF & WHIM & 0.8645 / 0.8864 & 0.8817 / 1.1043 & 0.7819 / 0.8769 & 0.8331 / 0.7674 & 1.2578 / 1.3597 & 1.0416 / 0.9957 & 1.0260 / 1.0795 & 0.8840 / 0.8941 & 0.9895 / 1.0222 & 1.0496 / 1.0408 \\
GBM & WHIM & 0.8732 / 0.8501 & 0.9027 / 1.1041 & 0.7699 / 0.8551 & 0.8528 / 0.7324 & 1.2664 / 1.3814 & 1.0032 / 0.9607 & 1.0479 / 1.0890 & 0.8906 / 0.9158 & 1.0327 / 1.0755 & 1.0791 / 1.0201 \\
SVM & WHIM & 1.0280 / 0.9655 & 0.8571 / 1.0881 & 0.8420 / 0.9637 & 0.8511 / 0.8248 & 1.3113 / 1.4359 & 1.1029 / 1.0025 & 1.0600 / 1.0669 & 0.8907 / 0.9255 & 1.0407 / 1.0740 & 1.0948 / 1.0355 \\
KNN & WHIM & 0.9865 / 0.8491 & 0.8810 / 1.0691 & 0.8047 / 0.9293 & 0.8407 / 0.8327 & 1.3652 / 1.4822 & 1.1407 / 1.0130 & 1.0693 / 1.1120 & 0.9208 / 0.9195 & 1.0611 / 1.0863 & 1.0756 / 1.0168 \\
MPNN & GRAPH & 0.9477 / 0.8884 & 1.0583 / 1.1539 & 0.9048 / 0.9268 & 1.0302 / 0.9509 & 1.4584 / 1.5806 & 1.0245 / 0.9340 & 1.1833 / 1.2433 & 1.0531 / 1.0623 & 0.9030 / 0.9193 & 0.9995 / 1.0145 \\
AFP & GRAPH & 1.3474 / 1.1578 & 1.1428 / 1.2745 & 0.9309 / 0.9486 & 0.9703 / 0.9023 & 1.5527 / 1.7434 & 1.9063 / 1.3681 & 1.0832 / 1.1343 & 1.0459 / 1.0402 & 0.9523 / 0.9656 & 1.1923 / 1.1603 \\
$\mathrm{MolCLR}_{\text{gcn}}$ & GRAPH & 0.9896 / 1.1098 & 0.9482 / 0.8629 & 1.3034 / 1.3151 & 0.7810 / 0.7568 & 1.5917 / 1.6165 & 1.5509 / 1.5455 & 1.0088 / 1.0386 & 1.0999 / 1.1056 & 0.9866 / 0.9428 & 1.3398 / 1.3170 \\
$\mathrm{MolCLR}^{\text{pretrained}}_{\text{gcn}}$ & GRAPH & 1.0680 / 1.1939 & 0.9248 / 0.8320 & 1.2919 / 1.3054 & 0.7672 / 0.7390 & 1.5568 / 1.5791 & 1.9046 / 2.0633 & 1.0503 / 1.0759 & 1.0720 / 1.1182 & 0.9838 / 0.9396 & 1.3396 / 1.3288 \\
PPNP & GRAPH & 1.4631 / 1.4367 & 1.1400 / 1.3332 & 1.0041 / 0.9308 & 1.2564 / 0.9284 & 1.5242 / 1.7086 & 1.9766 / 1.8805 & 1.1338 / 1.1517 & 1.0523 / 0.9986 & 1.0711 / 1.0656 & 1.1956 / 1.1603 \\
$\mathrm{MolCLR}^{\text{pretrained}}_{\text{gin}}$ & GRAPH & 1.0512 / 1.1760 & 1.0775 / 1.0196 & 1.5104 / 1.5500 & 0.7840 / 0.7643 & 1.6887 / 1.7093 & 1.2265 / 1.0147 & 1.1438 / 1.1834 & 1.0999 / 1.1056 & 1.0222 / 0.9912 & 1.4587 / 1.3643 \\
$\mathrm{MolCLR}_{\text{gin}}$ & GRAPH & 1.0512 / 1.1760 & 1.0775 / 1.0196 & 1.4538 / 1.4921 & 0.7840 / 0.7643 & 1.6887 / 1.7093 & 1.2265 / 1.0147 & 1.1438 / 1.1834 & 1.0697 / 1.0587 & 1.0222 / 0.9912 & 1.4587 / 1.3643 \\
$\mathrm{Contextpred}^{\text{pretrained}}$ & GRAPH & 1.3513 / 1.8131 & 1.7136 / 1.7663 & 1.4155 / 1.4123 & 1.6540 / 2.0069 & 1.9574 / 2.2021 & 1.2663 / 1.8716 & 1.5010 / 1.5931 & 1.7257 / 1.9468 & 1.6610 / 1.6946 & 1.4937 / 1.6573 \\
Contextpred & GRAPH & 1.3711 / 1.8173 & 1.6469 / 1.6866 & 1.4749 / 1.4535 & 1.7401 / 2.0606 & 2.0118 / 2.2692 & 1.2950 / 1.8566 & 1.6802 / 1.7679 & 1.5827 / 1.7777 & 1.6858 / 1.7417 & 1.6626 / 1.8030 \\
$\mathrm{KPGT}^{\text{pretrained}}$ & GRAPH & 1.6267 / 1.3956 & 1.9951 / 1.8846 & 1.4158 / 1.5493 & 2.8480 / 2.7568 & 2.2878 / 2.1817 & 1.6150 / 1.1296 & 1.7811 / 1.7774 & 2.3303 / 2.3055 & 1.9625 / 1.9738 & 1.8300 / 1.8475 \\
KPGT & GRAPH & 1.6682 / 1.4652 & 1.9764 / 1.8220 & 1.4203 / 1.5942 & 2.8369 / 2.6945 & 2.3020 / 2.2098 & 1.6755 / 1.2009 & 1.8017 / 1.7803 & 2.1985 / 2.0988 & 2.1214 / 2.0995 & 1.8556 / 1.8465 \\
\bottomrule
\end{tabular}

}
\label{tab:rmse_cliff_part1}
\end{table}

%\end{landscape}



==> tables/full_results2.tex <==
%\begin{landscape}
\begin{table}[htbp]
\centering
\caption{RMSE / $\text{RMSE}_{\text{cliff}}$ (Part 2/3) with best (\textbf{bold}) and second-best (\underline{underlined}) highlighted.}
\scalebox{0.73}{%
\begin{tabular}{llcccccccccc}
\toprule
\textbf{Algorithm} & \textbf{Descriptor} & \textbf{CHEMBL231} & \textbf{CHEMBL233} & \textbf{CHEMBL234} & \textbf{CHEMBL235} & \textbf{CHEMBL236} & \textbf{CHEMBL237} & \textbf{CHEMBL237} & \textbf{CHEMBL238} & \textbf{CHEMBL239} & \textbf{CHEMBL244} \\
& & \textbf{(Ki)} & \textbf{(Ki)} & \textbf{(Ki)} & \textbf{(EC50)} & \textbf{(Ki)} & \textbf{(EC50)} & \textbf{(Ki)} & \textbf{(Ki)} & \textbf{(EC50)} & \textbf{(Ki)} \\

\midrule
GraphCliff & GRAPH & \textbf{0.7080} / 0.8660 & 0.7860 / 0.8803 & \underline{0.6175} / \underline{0.6316} & 0.6504 / \textbf{0.7544} & 0.6965 / \underline{0.7850} & \textbf{0.7075} / \textbf{0.7668} & 0.7046 / 0.7833 & \textbf{0.5966} / 0.7293 & \textbf{0.6701} / \textbf{0.7919} & \textbf{0.6683} / \underline{0.7516} \\
GraphCliff w/ JK-Net & GRAPH & 0.7292 / 0.8745 & \textbf{0.7642} / 0.8663 & \textbf{0.5991} / \textbf{0.5979} & 0.6551 / \underline{0.7642} & \textbf{0.6873} / 0.7958 & 0.7294 / 0.8026 & \underline{0.6985} / \underline{0.7567} & 0.6102 / 0.7264 & \underline{0.6728} / \underline{0.8019} & 0.6830 / 0.7683 \\
SVM & ECFP & 0.7503 / 0.9322 & \underline{0.7742} / 0.8591 & 0.6217 / 0.6318 & \underline{0.6397} / 0.7743 & 0.6981 / 0.7978 & \underline{0.7200} / \underline{0.7816} & \textbf{0.6771} / \textbf{0.7350} & 0.6101 / 0.6808 & 0.6776 / 0.8191 & 0.7152 / 0.7966 \\
GraphCLiff w/ Residual & GRAPH & \underline{0.7155} / 0.8663 & 0.7929 / 0.8847 & 0.6331 / 0.6409 & 0.6513 / 0.7766 & 0.7023 / \textbf{0.7592} & 0.7776 / 0.8797 & 0.7174 / 0.7876 & \underline{0.6006} / 0.6958 & 0.7263 / 0.8391 & \underline{0.6826} / \textbf{0.7485} \\
GBM & ECFP & 0.7737 / 0.9548 & 0.8017 / 0.8857 & 0.6293 / 0.6486 & 0.6631 / 0.8063 & \underline{0.6962} / 0.7935 & 0.8026 / 0.8803 & 0.7127 / 0.7887 & 0.6180 / \textbf{0.6377} & 0.6825 / 0.8205 & 0.7361 / 0.8208 \\
RF & ECFP & 0.8215 / 0.9074 & 0.8007 / 0.8796 & 0.6600 / 0.6829 & \textbf{0.6385} / 0.7644 & 0.7108 / 0.7921 & 0.7620 / 0.7927 & 0.7288 / 0.7995 & 0.6247 / \underline{0.6562} & 0.6890 / 0.8248 & 0.7407 / 0.8231 \\
GINE + PairNorm & GRAPH & 0.7292 / 0.7855 & 0.7959 / 0.8899 & 0.6819 / 0.7028 & 0.6473 / 0.7946 & 0.7575 / 0.8165 & 0.7571 / 0.8735 & 0.7384 / 0.8103 & 0.6578 / 0.7359 & 0.7331 / 0.8636 & 0.7861 / 0.8591 \\
JK-Net & GRAPH & 0.7756 / 0.8577 & 0.7766 / 0.8589 & 0.6553 / 0.6557 & 0.6716 / 0.7849 & 0.7412 / 0.8329 & 0.7637 / 0.8654 & 0.7474 / 0.8238 & 0.6437 / 0.7385 & 0.7858 / 0.9106 & 0.7580 / 0.8343 \\
GINE + NodeNorm & GRAPH & 0.7566 / 0.8443 & 0.7912 / 0.8769 & 0.6717 / 0.6545 & 0.6563 / 0.7793 & 0.7300 / 0.8169 & 0.7381 / 0.8174 & 0.7279 / 0.7953 & 0.6663 / 0.7469 & 0.6928 / 0.8229 & 0.7576 / 0.8361 \\
GINE + Residual & GRAPH & 0.7953 / 0.8026 & 0.7937 / 0.8812 & 0.6940 / 0.6995 & 0.6882 / 0.8191 & 0.7357 / 0.7980 & 0.7709 / 0.8544 & 0.7528 / 0.8101 & 0.7026 / 0.7650 & 0.7095 / 0.8393 & 0.7655 / 0.8153 \\
KNN & ECFP & 0.7763 / 1.0202 & 0.8160 / 0.9123 & 0.6752 / 0.6989 & 0.6881 / 0.7946 & 0.7458 / 0.8650 & 0.8100 / 0.8758 & 0.7362 / 0.8507 & 0.6466 / 0.7346 & 0.7136 / 0.8646 & 0.7674 / 0.8735 \\
ChemProp & GRAPH & 0.7596 / 0.8169 & 0.7990 / \underline{0.8438} & 0.6868 / 0.6532 & 0.7081 / 0.7995 & 0.7992 / 0.8827 & 0.7674 / 0.8394 & 0.7426 / 0.8003 & 0.6730 / 0.7361 & 0.8194 / 0.8271 & 0.7256 / 0.7972 \\
LSTM & SMILES & 0.8086 / 1.0703 & 0.8501 / 0.9418 & 0.7381 / 0.7970 & 0.7270 / 0.8474 & 0.8118 / 0.9051 & 0.7832 / 0.9028 & 0.7735 / 0.8618 & 0.6536 / 0.7925 & 0.7648 / 0.9051 & 0.8003 / 0.9128 \\
GBM & MACCS & 0.7543 / \underline{0.7590} & 0.8463 / 0.9134 & 0.7189 / 0.7241 & 0.7131 / 0.8604 & 0.8392 / 0.9308 & 0.8312 / 0.9041 & 0.7994 / 0.8857 & 0.6783 / 0.6999 & 0.7207 / 0.8409 & 0.7989 / 0.8789 \\
SVM & MACCS & 0.7829 / 0.8372 & 0.8685 / 0.9534 & 0.7392 / 0.7293 & 0.6961 / 0.8382 & 0.8498 / 0.9377 & 0.8316 / 0.8853 & 0.7791 / 0.8726 & 0.6687 / 0.6821 & 0.7178 / 0.8533 & 0.8183 / 0.8697 \\
RF & MACCS & 0.7386 / 0.8280 & 0.8284 / 0.9060 & 0.7443 / 0.7498 & 0.7052 / 0.8232 & 0.8281 / 0.9565 & 0.8488 / 0.9113 & 0.8140 / 0.9274 & 0.7024 / 0.7082 & 0.7346 / 0.8681 & 0.8458 / 0.9174 \\
MLP & ECFP & 1.3335 / 1.2722 & 0.8452 / 0.9157 & 0.6693 / 0.6759 & 0.7180 / 0.8178 & 0.7329 / 0.8098 & 0.9018 / 0.9504 & 0.7216 / 0.7653 & 0.6839 / 0.7320 & 0.7559 / 0.9010 & 0.7955 / 0.8497 \\
GINE + DropEdge & GRAPH & 0.7923 / 0.8716 & 0.8611 / 0.9405 & 0.7518 / 0.7418 & 0.7117 / 0.8541 & 0.8138 / 0.9103 & 0.8950 / 0.9487 & 0.7821 / 0.8438 & 0.7444 / 0.8308 & 0.7924 / 0.9296 & 0.8467 / 0.9104 \\
SCAGE & GRAPH & 0.9145 / 0.7844 & 0.8244 / \textbf{0.8004} & 0.7993 / 0.8114 & 0.6941 / 0.7875 & 0.7987 / 0.9285 & 0.9673 / 0.9601 & 0.7623 / 0.8222 & 0.7261 / 0.6813 & 0.7959 / 0.8506 & 0.8923 / 0.9723 \\
GCNII & GRAPH & 0.8574 / 0.7778 & 0.8372 / 0.9122 & 0.7294 / 0.7103 & 0.6928 / 0.8318 & 0.7863 / 0.8299 & 1.0908 / 1.0403 & 0.7692 / 0.8311 & 0.7274 / 0.7441 & 0.7561 / 0.8674 & 0.8574 / 0.9347 \\
KNN & MACCS & 0.8366 / 0.9586 & 0.8523 / 0.9106 & 0.7817 / 0.7580 & 0.7503 / 0.8682 & 0.8963 / 1.0465 & 0.9619 / 0.9503 & 0.8249 / 0.9426 & 0.7077 / 0.7353 & 0.7910 / 0.8951 & 0.9016 / 0.9473 \\
APPNP & GRAPH & 0.8659 / 0.8776 & 0.9045 / 0.9578 & 0.7938 / 0.7788 & 0.7608 / 0.9047 & 0.8622 / 0.9159 & 0.9286 / 0.9318 & 0.8286 / 0.8655 & 0.7846 / 0.8673 & 0.8233 / 0.9480 & 0.9900 / 0.9899 \\
RF & PHYSCHEM & 0.9078 / \textbf{0.7321} & 1.0193 / 0.9963 & 0.8866 / 0.8586 & 0.7949 / 0.8915 & 0.9893 / 0.9983 & 0.9660 / 0.8935 & 0.9612 / 0.9795 & 0.9034 / 0.8508 & 0.8839 / 1.0317 & 1.1161 / 1.1190 \\
GBM & PHYSCHEM & 0.9531 / 0.8270 & 1.0502 / 1.0373 & 0.8832 / 0.8464 & 0.8210 / 0.9114 & 1.0141 / 1.0165 & 0.9992 / 0.9420 & 0.9609 / 0.9688 & 0.9018 / 0.8363 & 0.8745 / 1.0227 & 1.1047 / 1.1251 \\
Transformer & TOKENS & 0.9641 / 1.0284 & 1.0720 / 1.1179 & 0.8626 / 0.8483 & 0.8015 / 0.9136 & 1.0236 / 1.1023 & 1.1260 / 1.1842 & 0.9961 / 1.0624 & 0.8802 / 0.8515 & 0.9095 / 1.0319 & 1.0781 / 1.0707 \\
GCN & GRAPH & 0.8783 / 0.7969 & 1.0561 / 1.1056 & 0.9344 / 0.9186 & 0.9008 / 1.0389 & 0.9425 / 1.0003 & 1.1316 / 1.0944 & 1.1119 / 1.1521 & 0.9370 / 0.9249 & 0.9055 / 1.0237 & 1.0745 / 1.0602 \\
KNN & PHYSCHEM & 1.0454 / 0.8996 & 1.0372 / 1.0296 & 0.9109 / 0.8977 & 0.8736 / 0.9376 & 1.0324 / 1.0278 & 0.9983 / 0.9304 & 0.9686 / 0.9554 & 0.9394 / 0.8525 & 0.8738 / 0.9912 & 1.1384 / 1.1425 \\
CNN & SMILES & 1.0080 / 1.0442 & 1.0730 / 1.0796 & 0.8979 / 0.8811 & 0.8925 / 0.9623 & 1.0179 / 1.0669 & 1.0608 / 1.0216 & 1.0401 / 1.0403 & 0.9175 / 0.8975 & 0.9102 / 0.9857 & 1.0945 / 1.0706 \\
SVM & PHYSCHEM & 0.9936 / 0.8922 & 1.1595 / 1.1296 & 0.9436 / 0.8892 & 0.9126 / 1.0058 & 1.1155 / 1.2229 & 1.0847 / 1.0709 & 1.0199 / 1.0438 & 1.0011 / 0.9546 & 0.9641 / 1.0548 & 1.1602 / 1.1158 \\
GAT & GRAPH & 0.9909 / 0.9696 & 1.0659 / 1.0986 & 0.9499 / 0.9119 & 0.8692 / 1.0117 & 1.0023 / 1.0999 & 1.1029 / 1.0637 & 1.0850 / 1.0978 & 0.9276 / 0.9458 & 0.9016 / 1.0123 & 1.0881 / 1.1173 \\
RF & WHIM & 0.9533 / 0.9391 & 1.1316 / 1.1480 & 0.9691 / 0.9023 & 1.0037 / 1.1015 & 1.1178 / 1.1631 & 1.3018 / 1.3140 & 1.1205 / 1.1400 & 0.9935 / 0.9634 & 0.9979 / 1.0783 & 1.2490 / 1.2071 \\
GBM & WHIM & 0.9591 / 0.9619 & 1.1469 / 1.1585 & 0.9991 / 0.9123 & 1.0001 / 1.1008 & 1.1319 / 1.1788 & 1.3569 / 1.3497 & 1.1247 / 1.1285 & 0.9907 / 0.9495 & 1.0475 / 1.1333 & 1.2866 / 1.2301 \\
SVM & WHIM & 0.9558 / 0.9001 & 1.1497 / 1.1909 & 0.9871 / 0.9221 & 0.9920 / 1.0815 & 1.1393 / 1.2000 & 1.3074 / 1.2991 & 1.1750 / 1.2217 & 0.9733 / 0.9897 & 1.0164 / 1.1355 & 1.3053 / 1.2769 \\
KNN & WHIM & 1.0074 / 0.9088 & 1.1947 / 1.2158 & 1.0171 / 0.9445 & 0.9782 / 1.0792 & 1.1499 / 1.2141 & 1.3190 / 1.3189 & 1.1743 / 1.1873 & 1.0473 / 1.0123 & 1.0187 / 1.1004 & 1.2742 / 1.2174 \\
MPNN & GRAPH & 1.3047 / 1.2233 & 1.0740 / 1.1382 & 0.9586 / 0.9216 & 1.0579 / 1.1940 & 1.3639 / 1.4539 & 1.4020 / 1.3336 & 1.0528 / 1.1094 & 1.1417 / 1.2077 & 1.2883 / 1.4815 & 1.6595 / 1.5569 \\
AFP & GRAPH & 1.2615 / 1.1557 & 1.2106 / 1.2335 & 0.8850 / 0.8642 & 1.2019 / 1.3078 & 1.3705 / 1.4229 & 1.3606 / 1.3041 & 1.3104 / 1.4115 & 1.2157 / 1.2252 & 1.3611 / 1.5731 & 1.7060 / 1.5913 \\
$\mathrm{MolCLR}_{\text{gcn}}$  & GRAPH & 1.2319 / 1.2398 & 1.2528 / 1.2835 & 1.2779 / 1.2919 & 1.0446 / 1.0717 & 1.3564 / 1.3406 & 1.1112 / 1.1396 & 1.3807 / 1.4115 & 1.1568 / 1.2928 & 0.9683 / 1.0252 & 1.8312 / 1.8374 \\
$\mathrm{MolCLR}^{\text{pretrained}}_{\text{gcn}}$  & GRAPH & 1.3950 / 1.4198 & 1.2290 / 1.2562 & 1.3255 / 1.3353 & 1.0275 / 1.0452 & 1.3146 / 1.2956 & 1.2088 / 1.2518 & 1.3378 / 1.3655 & 1.1677 / 1.3067 & 0.9439 / 0.9968 & 1.8971 / 1.9297 \\
PPNP & GRAPH & 1.3204 / 1.2262 & 1.2973 / 1.3029 & 1.1354 / 1.0602 & 1.0675 / 1.1460 & 1.3322 / 1.3214 & 1.4430 / 1.3491 & 1.3400 / 1.4205 & 1.1516 / 1.1805 & 1.0983 / 1.1795 & 1.6043 / 1.5392 \\
$\mathrm{MolCLR}^{\text{pretrained}}_{\text{gin}}$  & GRAPH & 1.6430 / 1.6588 & 1.2987 / 1.3599 & 1.3471 / 1.3572 & 1.3126 / 1.3911 & 1.4144 / 1.3823 & 1.0887 / 1.1027 & 1.3450 / 1.3897 & 1.1978 / 1.3359 & 1.0543 / 1.1123 & 1.8490 / 1.8369 \\
$\mathrm{MolCLR}_{\text{gin}}$  & GRAPH & 1.6430 / 1.6588 & 1.3137 / 1.3302 & 1.3471 / 1.3572 & 1.3126 / 1.3911 & 1.4144 / 1.3823 & 1.0887 / 1.1027 & 1.4369 / 1.4828 & 1.1978 / 1.3359 & 1.0543 / 1.1123 & 1.8490 / 1.8369 \\
$\mathrm{Contextpred}^{\text{pretrained}}$ & GRAPH & 1.9750 / 2.1353 & 1.8107 / 1.9078 & 1.3493 / 1.4886 & 1.6154 / 1.8623 & 1.4829 / 1.7134 & 1.6653 / 1.7664 & 1.5641 / 1.7102 & 1.6095 / 2.0372 & 1.8364 / 2.0995 & 1.8936 / 2.0112 \\
Contextpred & GRAPH & 1.8816 / 1.9981 & 1.8158 / 1.9027 & 1.4666 / 1.5984 & 1.7811 / 1.9887 & 1.6644 / 1.9059 & 1.7069 / 1.8184 & 1.6768 / 1.8274 & 1.6665 / 2.0558 & 1.8929 / 2.1681 & 1.9221 / 2.0561 \\
$\mathrm{KPGT}^{\text{pretrained}}$ & GRAPH & 2.2765 / 2.4227 & 1.8560 / 1.8244 & 1.6561 / 1.6645 & 2.6720 / 2.6705 & 2.1335 / 2.0196 & 1.7889 / 1.8235 & 1.8541 / 1.8355 & 2.4356 / 2.3289 & 2.7528 / 2.6857 & 2.0671 / 2.0234 \\
KPGT & GRAPH & 2.6051 / 2.6221 & 1.6700 / 1.6562 & 1.6763 / 1.7084 & 2.6704 / 2.6356 & 2.1538 / 2.0568 & 1.6908 / 1.7617 & 2.1583 / 2.0943 & 2.3888 / 2.2401 & 2.7510 / 2.6604 & 2.1260 / 2.1025 \\
\bottomrule
\end{tabular}%
}
\label{tab:rmse_cliff_part2}
\end{table}
%\end{landscape}

==> tables/full_results3.tex <==
%\begin{landscape}
\begin{table}[htbp]
\centering
\caption{RMSE / $\text{RMSE}_{\text{cliff}}$ (Part 3/3) with best (\textbf{bold}) and second-best (\underline{underlined}) highlighted.}
\scalebox{0.73}{%
\begin{tabular}{llcccccccccc}
\toprule
\textbf{Algorithm} & \textbf{Descriptor} & \textbf{CHEMBL262} & \textbf{CHEMBL264} & \textbf{CHEMBL2835} & \textbf{CHEMBL287} & \textbf{CHEMBL2971} & \textbf{CHEMBL3979} & \textbf{CHEMBL4005} & \textbf{CHEMBL4203} & \textbf{CHEMBL4616} & \textbf{CHEMBL4792} \\
& & \textbf{(Ki)} & \textbf{(Ki)} & \textbf{(Ki)} & \textbf{(Ki)} & \textbf{(Ki)} & \textbf{(EC50)} & \textbf{(Ki)} & \textbf{(Ki)} & \textbf{(EC50)} & \textbf{(Ki)} \\
\midrule
GraphCliff & GRAPH & 0.7523 / \underline{0.7019} & \underline{0.6189} / \underline{0.6715} & 0.3959 / 0.7953 & 0.7055 / 0.7977 & 0.6154 / 0.7777 & \textbf{0.6226} / \textbf{0.6536} & \textbf{0.6174} / \textbf{0.7122} & 0.8999 / 1.1768 & \textbf{0.6342} / 0.7186 & 0.6351 / \underline{0.6513} \\
GraphCliff w/ JK-Net & GRAPH & \textbf{0.7108} / 0.7118 & 0.6424 / 0.6957 & 0.3986 / 0.8506 & \textbf{0.7016} / 0.7356 & \textbf{0.5893} / 0.7058 & 0.6635 / 0.7087 & 0.6516 / 0.7400 & \underline{0.8724} / 1.1417 & 0.6631 / 0.7244 & 0.6401 / 0.6595 \\
SVM & ECFP & 0.7236 / \textbf{0.6556} & \textbf{0.6150} / 0.6741 & 0.4198 / 0.7427 & 0.7142 / 0.8115 & \underline{0.6050} / 0.6590 & \underline{0.6295} / \underline{0.6737} & 0.6462 / 0.7415 & 0.8798 / \textbf{1.0014} & \underline{0.6353} / \underline{0.6924} & \underline{0.6334} / \textbf{0.6381} \\
GraphCLiff w/ Residual & GRAPH & 0.7886 / 0.9097 & 0.6488 / 0.7051 & 0.3903 / 0.8178 & 0.7363 / 0.8150 & 0.6695 / 0.7589 & 0.6951 / 0.7653 & 0.6386 / \underline{0.7277} & \textbf{0.8198} / 1.0360 & 0.6973 / 0.7425 & \textbf{0.6332} / 0.6818 \\
GBM & ECFP & 0.7498 / 0.7274 & 0.6486 / 0.7215 & 0.4053 / 0.7893 & 0.7591 / 0.8473 & 0.6157 / 0.6667 & 0.6595 / 0.7217 & 0.6468 / 0.7482 & 0.9194 / 1.0753 & 0.6857 / 0.7675 & 0.6737 / 0.6865 \\
RF & ECFP & \underline{0.7212} / 0.7749 & 0.6586 / 0.7418 & \underline{0.3876} / 0.8021 & 0.7758 / 0.8911 & 0.6297 / \textbf{0.6428} & 0.6497 / 0.7078 & 0.6475 / 0.7321 & 0.8816 / 1.0809 & 0.6816 / 0.7695 & 0.7086 / 0.7211 \\
GINE+PairNorm & GRAPH & 0.7891 / 0.9355 & 0.6431 / 0.7241 & \textbf{0.3840} / 0.7499 & 0.7338 / 0.7459 & 0.6835 / 0.8511 & 0.6308 / 0.6898 & 0.6671 / 0.7668 & 0.9310 / 1.2276 & 0.6916 / 0.7698 & 0.6760 / 0.6968 \\
JK-Net & GRAPH & 0.8369 / 0.8611 & 0.6578 / 0.7186 & 0.4208 / 0.7796 & \underline{0.7023} / \underline{0.7269} & 0.6544 / 0.7893 & 0.6838 / 0.7149 & \underline{0.6221} / 0.7734 & 0.9765 / 1.0937 & 0.7140 / 0.7502 & 0.6805 / 0.6948 \\
GINE+NodeNorm & GRAPH & 0.8071 / 0.8037 & 0.6582 / 0.7159 & 0.4147 / 0.7563 & 0.7331 / 0.7663 & 0.6468 / 0.7698 & 0.6894 / 0.7025 & 0.6738 / 0.7833 & 0.9556 / 1.2305 & 0.6746 / 0.6998 & 0.7496 / 0.7339 \\
GINE+Residual & GRAPH & 0.8593 / 0.8792 & 0.6628 / 0.7499 & 0.4287 / 0.8235 & 0.7421 / 0.7571 & 0.6921 / 0.7991 & 0.6784 / 0.7153 & 0.6498 / 0.7412 & 0.9403 / 1.2689 & 0.6603 / 0.7098 & 0.7617 / 0.7714 \\
KNN & ECFP & 0.8337 / 0.8994 & 0.6739 / 0.8053 & 0.4362 / 0.8584 & 0.8100 / 0.9569 & 0.6634 / 0.7824 & 0.6836 / 0.7389 & 0.6557 / 0.7540 & 0.9718 / 1.0740 & 0.7398 / 0.8282 & 0.6955 / 0.7244 \\
ChemProp & GRAPH & 0.8680 / 1.0281 & 0.6368 / \textbf{0.6520} & 0.4331 / 0.7623 & 0.7086 / \textbf{0.7153} & 0.7445 / 0.9535 & 0.7108 / 0.7705 & 0.7088 / 0.8083 & 1.0027 / 1.4844 & 0.7036 / 0.7947 & 0.6751 / 0.7131 \\
LSTM & SMILES & 0.7672 / 0.7814 & 0.6652 / 0.7666 & 0.4314 / 0.8404 & 0.7913 / 0.8942 & 0.6887 / 0.8860 & 0.7404 / 0.7903 & 0.7637 / 0.9005 & 0.9071 / 1.3177 & 0.7392 / 0.8308 & 0.6910 / 0.7499 \\
GBM & MACCS & 0.8090 / 0.8785 & 0.6960 / 0.7901 & 0.4807 / 0.9261 & 0.7876 / 0.8361 & 0.6585 / \underline{0.6456} & 0.6611 / 0.7034 & 0.6755 / 0.7899 & 0.9836 / 1.4244 & 0.7151 / 0.7949 & 0.7564 / 0.7935 \\
SVM & MACCS & 0.8339 / 0.9592 & 0.7205 / 0.8131 & 0.4643 / 0.7648 & 0.7380 / 0.7890 & 0.6568 / 0.6987 & 0.6728 / 0.7146 & 0.7233 / 0.8439 & 0.9817 / 1.4668 & 0.7173 / 0.7795 & 0.7488 / 0.7798 \\
RF & MACCS & 0.8847 / 0.8843 & 0.7379 / 0.8311 & 0.4372 / 0.8238 & 0.7891 / 0.8333 & 0.6369 / 0.6565 & 0.6963 / 0.7267 & 0.7013 / 0.8448 & 0.9292 / 1.3265 & 0.7168 / 0.7721 & 0.7867 / 0.8266 \\
MLP & ECFP & 0.9041 / 0.9484 & 0.6719 / 0.7309 & 0.4878 / 0.8757 & 0.7325 / 0.8519 & 0.6743 / 0.7636 & 0.6610 / 0.7244 & 0.6798 / 0.7694 & 0.9468 / 1.0265 & 0.7268 / 0.7779 & 0.6915 / 0.6821 \\
GINE+DropEdge & GRAPH & 0.9186 / 0.8750 & 0.7444 / 0.7897 & 0.4785 / 0.9170 & 0.8330 / 0.8733 & 0.6790 / 0.8311 & 0.7519 / 0.7878 & 0.7042 / 0.8006 & 0.9499 / 1.1955 & 0.7476 / 0.7609 & 0.8374 / 0.8613 \\
SCAGE & GRAPH & 0.9228 / 0.8449 & 0.7048 / 0.7383 & 0.5052 / 0.6936 & 0.8011 / 0.8126 & 0.7453 / 0.7260 & 0.9212 / 0.8939 & 0.7048 / 0.7698 & 1.0241 / \underline{1.0160} & 0.7396 / \textbf{0.6857} & 0.7808 / 0.8590 \\
GCNII & GRAPH & 0.9118 / 0.9378 & 0.7039 / 0.7747 & 0.4760 / 0.9362 & 0.8044 / 0.8662 & 0.8598 / 0.8850 & 0.7640 / 0.7988 & 0.8057 / 0.8503 & 0.9767 / 1.1498 & 0.7375 / 0.7396 & 0.7916 / 0.8003 \\
KNN & MACCS & 0.9168 / 1.1287 & 0.7698 / 0.8905 & 0.4669 / 0.8819 & 0.8423 / 0.9244 & 0.7316 / 0.6706 & 0.7069 / 0.7492 & 0.7657 / 0.8732 & 1.0308 / 1.5023 & 0.7113 / 0.7821 & 0.8627 / 0.8859 \\
APPNP & GRAPH & 0.9799 / 0.9536 & 0.7942 / 0.8439 & 0.5020 / 0.9794 & 0.7939 / 0.8640 & 0.8402 / 0.8530 & 0.8222 / 0.7956 & 0.7212 / 0.8305 & 1.0061 / 1.2026 & 0.7972 / 0.7732 & 0.8115 / 0.8130 \\
RF & PHYSCHEM & 0.8634 / 0.8645 & 0.8511 / 0.8861 & 0.5017 / 0.8914 & 0.7844 / 0.7866 & 0.8153 / 0.7967 & 0.8731 / 0.8188 & 0.8000 / 0.9034 & 1.0024 / 1.4555 & 0.8165 / 0.8403 & 0.8440 / 0.8257 \\
GBM & PHYSCHEM & 0.8746 / 0.9121 & 0.8779 / 0.9155 & 0.5389 / 0.9050 & 0.8057 / 0.8152 & 0.8588 / 0.8879 & 0.8673 / 0.7997 & 0.7819 / 0.8625 & 1.0136 / 1.5379 & 0.8280 / 0.8525 & 0.8464 / 0.8221 \\
Transformer & TOKENS & 0.9765 / 1.0519 & 0.8221 / 0.8820 & 0.4850 / 0.7722 & 0.8694 / 0.9269 & 0.8262 / 0.9542 & 0.8335 / 0.8804 & 0.8546 / 0.9406 & 0.9594 / 1.1445 & 0.7842 / 0.8165 & 0.9124 / 0.9113 \\
GCN & GRAPH & 0.9337 / 1.0044 & 0.8553 / 0.9102 & 0.5052 / 0.9256 & 0.8861 / 0.9000 & 0.7806 / 0.9167 & 0.8120 / 0.8047 & 0.8752 / 0.9087 & 0.9747 / 1.2114 & 0.8674 / 0.8306 & 0.9226 / 0.9264 \\
KNN & PHYSCHEM & 0.9064 / 0.9357 & 0.8786 / 0.9003 & 0.4907 / 0.8244 & 0.8490 / 0.8381 & 0.7766 / 0.7524 & 0.9549 / 0.8427 & 0.8197 / 0.8410 & 0.9828 / 1.3259 & 0.8384 / 0.8566 & 0.9096 / 0.8561 \\
CNN & SMILES & 0.9477 / 0.9534 & 0.8901 / 0.9151 & 0.5596 / 0.8712 & 0.8908 / 0.9212 & 0.8311 / 0.8609 & 0.9074 / 0.8588 & 0.8381 / 0.9279 & 1.0128 / 1.2306 & 0.8190 / 0.8207 & 0.9673 / 0.9662 \\
SVM & PHYSCHEM & 0.9489 / 1.0021 & 0.9085 / 0.9167 & 0.4135 / \textbf{0.6398} & 0.8179 / 0.8092 & 0.9504 / 0.8548 & 0.9186 / 0.8843 & 0.7993 / 0.8523 & 1.0052 / 1.2213 & 0.8413 / 0.8255 & 0.8697 / 0.8703 \\
GAT & GRAPH & 0.9943 / 1.0323 & 0.8958 / 0.9356 & 0.5554 / 0.9240 & 0.9470 / 0.9944 & 0.8026 / 0.9663 & 0.9232 / 0.9139 & 0.8613 / 0.9013 & 1.0039 / 1.2080 & 0.8734 / 0.8351 & 1.0036 / 1.0141 \\
RF & WHIM & 0.9294 / 1.0229 & 0.9363 / 0.9698 & 0.4783 / 0.7437 & 0.9168 / 1.0236 & 0.7499 / 0.8256 & 0.9965 / 0.9384 & 0.8845 / 0.9045 & 0.9974 / 1.1101 & 0.9122 / 0.8879 & 1.0399 / 1.0222 \\
GBM & WHIM & 0.9356 / 1.0257 & 0.9700 / 1.0206 & 0.5030 / 0.7909 & 0.9407 / 1.0316 & 0.7812 / 0.8209 & 1.0372 / 0.9752 & 0.8817 / 0.9400 & 1.0340 / 1.2519 & 0.9515 / 0.9042 & 1.0398 / 1.0337 \\
SVM & WHIM & 0.8984 / 0.9927 & 0.9743 / 1.0097 & 0.5116 / 0.8028 & 0.9465 / 1.0426 & 0.8666 / 0.9746 & 1.0445 / 1.0198 & 0.9007 / 0.9405 & 1.0251 / 1.1688 & 0.9100 / 0.9003 & 1.0910 / 1.0968 \\
KNN & WHIM & 0.9133 / 0.8676 & 0.9742 / 1.0089 & 0.5335 / 0.9013 & 0.9741 / 1.0728 & 0.8099 / 0.8314 & 1.0187 / 0.9775 & 0.9285 / 0.9975 & 1.0704 / 1.3052 & 0.8847 / 0.8458 & 1.0522 / 1.0205 \\
MPNN & GRAPH & 1.0213 / 1.0356 & 1.0822 / 1.0124 & 0.6679 / 1.0670 & 0.9267 / 0.9732 & 0.9727 / 0.9446 & 1.1831 / 1.1452 & 0.9978 / 1.0160 & 1.0564 / 1.1486 & 0.9345 / 0.8603 & 1.1221 / 1.1141 \\
AFP & GRAPH & 1.1158 / 1.1835 & 1.1024 / 1.0617 & 0.7473 / 1.1064 & 1.1485 / 1.2151 & 1.0907 / 1.1009 & 1.0797 / 0.9897 & 1.0592 / 1.0789 & 1.0617 / 1.1308 & 0.9467 / 0.8722 & 1.2335 / 1.2376 \\
$\mathrm{MolCLR}_{\text{gcn}}$  & GRAPH & 1.2110 / 1.1067 & 1.0812 / 1.0247 & 1.1784 / 0.9831 & 0.8821 / 0.8618 & 1.7887 / 1.7890 & 1.0663 / 0.9434 & 1.0722 / 1.0537 & 1.0671 / 1.4879 & 0.9018 / 0.8160 & 1.2255 / 1.2214 \\
$\mathrm{MolCLR}^{\text{pretrained}}_{\text{gcn}}$  & GRAPH & 1.2197 / 1.0901 & 1.0675 / 1.0304 & 1.3432 / 1.1817 & 0.8728 / 0.8503 & 1.8176 / 1.8397 & 1.0532 / 0.9213 & 1.0446 / 1.0433 & 1.0725 / 1.5024 & 0.8989 / 0.8162 & 1.3483 / 1.3562 \\
PPNP & GRAPH & 1.0920 / 1.1605 & 1.0769 / 1.0153 & 0.9767 / 1.3259 & 1.0419 / 1.1170 & 1.3838 / 1.3053 & 1.1359 / 1.0032 & 1.0788 / 1.0877 & 1.0695 / 1.0985 & 0.9291 / 0.8418 & 1.1759 / 1.1685 \\
$\mathrm{MolCLR}^{\text{pretrained}}_{\text{gin}}$  & GRAPH & 1.1739 / 1.0662 & 1.0812 / 1.0247 & 1.0659 / 0.9023 & 0.8728 / 0.8503 & 1.2315 / 1.1016 & 0.9871 / 0.8284 & 1.1207 / 1.1324 & 1.0580 / 1.4872 & 0.9090 / 0.8243 & 1.4978 / 1.4986 \\
$\mathrm{MolCLR}_{\text{gin}}$  & GRAPH & 1.1739 / 1.0662 & 1.1757 / 1.1259 & 1.0659 / 0.9023 & 1.0022 / 0.9877 & 1.2315 / 1.1016 & 0.9871 / 0.8284 & 1.1207 / 1.1324 & 1.0345 / 1.4518 & 0.9604 / 0.8568 & 1.4978 / 1.4986 \\
$\mathrm{Contextpred}^{\text{pretrained}}$ & GRAPH & 1.9809 / 2.0611 & 1.6605 / 1.5609 & 1.5424 / 1.0246 & 1.5156 / 1.5724 & 1.7642 / 1.6268 & 1.6231 / 1.8675 & 1.5573 / 1.4940 & 1.7366 / 2.0266 & 1.2383 / 1.3317 & 1.7062 / 1.7833 \\
Contextpred & GRAPH & 1.9713 / 2.0586 & 1.5504 / 1.4692 & 1.6920 / 1.1823 & 1.3156 / 1.3855 & 1.4843 / 1.4337 & 1.7480 / 1.9870 & 1.5978 / 1.5115 & 1.9036 / 2.0851 & 1.6043 / 1.6481 & 1.7222 / 1.8009 \\
$\mathrm{KPGT}^{\text{pretrained}}$ & GRAPH & 2.6248 / 2.7108 & 1.3685 / 1.4650 & 0.5715 / 0.7474 & 1.6315 / 1.6767 & 1.3323 / 1.4566 & 2.3793 / 2.3392 & 1.5268 / 1.6350 & 2.5748 / 2.7290 & 1.3843 / 1.4016 & 2.1907 / 2.1513 \\
KPGT & GRAPH & 2.5337 / 2.6635 & 1.5136 / 1.5888 & 0.6072 / \underline{0.6824} & 1.4728 / 1.5559 & 1.3366 / 1.4283 & 2.1415 / 2.0541 & 1.5060 / 1.5896 & 2.5364 / 2.6396 & 1.4745 / 1.4685 & 2.3039 / 2.2114 \\
\bottomrule
\end{tabular}%
}
\label{tab:rmse_cliff_part3}
\end{table}
%\end{landscape}
